Neural Network Approximations of PDEs Beyond Linearity: A Representational Perspective

A burgeoning line of research leverages deep neural networks to approximate the solutions to high dimensional PDEs, opening lines of theoretical inquiry focused on explaining how it is that these models appear to evade the curse of dimensionality. However, most prior theoretical analyses have been limited to linear PDEs. In this work, we take a step towards studying the representational power of neural networks for approximating solutions to nonlinear PDEs. We focus on a class of PDEs known as \emph{nonlinear elliptic variational PDEs}, whose solutions minimize an \emph{Euler-Lagrange} energy functional $\mathcal{E}(u) = \int_\Omega L(x, u(x), \nabla u(x)) - f(x) u(x)dx$. We show that if composing a function with Barron norm $b$ with partial derivatives of $L$ produces a function of Barron norm at most $B_L b^p$, the solution to the PDE can be $\epsilon$-approximated in the $L^2$ sense by a function with Barron norm $O\left(\left(dB_L\right)^{\max\{p \log(1/ \epsilon), p^{\log(1/\epsilon)}\}}\right)$. By a classical result due to Barron [1993], this correspondingly bounds the size of a 2-layer neural network needed to approximate the solution. Treating $p, \epsilon, B_L$ as constants, this quantity is polynomial in dimension, thus showing neural networks can evade the curse of dimensionality. Our proof technique involves neurally simulating (preconditioned) gradient in an appropriate Hilbert space, which converges exponentially fast to the solution of the PDE, and such that we can bound the increase of the Barron norm at each iterate. Our results subsume and substantially generalize analogous prior results for linear elliptic PDEs over a unit hypercube.

==> icml2023/Scratchwork/General_form_of_L.tex <==
\section{Scratchwork}

\begin{definition}[Energy functional]
    \label{def:energy_functional}
    For all $u: \Omega \to \R$ such that $u|_{\partial \Omega} = 0$,
    we consider an energy functional of the following form:
    \begin{equation}
        \label{eq:main_energy_functional}
        \calE(u) = \int_\Omega \bigg(L(x, u(x), \nabla u(x)) - f(x) u(x)\bigg) dx,
    \end{equation}
    where $L : \R^{2d + 1}\to \R$ is a function that is strongly convex w.r.t $\nabla u(x)$,
    i.e., 
    there exists constant $0 < \lambda \leq \Lambda$
    such that for all $x \in \R$
    we have
    $\lambda I_d \leq \Dnbux L(x) \leq \Lambda I_d$. 
    Further, the function $L$ is convex w.r.t $u(x)$, i.e., we have
    $0 \leq \Dux L(x, u, \nabla u) \leq \varsigma$, where $\varsigma > 0$.
\end{definition}


\begin{proof}[Proof of Lemma~\ref{lemma:derivation_of_nonlinear_variational_PDE}]
    If the function $u^\star$ minimizes the energy functional in Definition \ref{def:energy_functional}
    then we have for all $\epsilon \in \R$
    $$ \calE(u) \leq \calE(u + \epsilon \varphi)$$
    where $\varphi \in C^\infty_c(\Omega)$.
    That is, we have a minima at $\epsilon = 0$ and taking a derivative w.r.t $\epsilon$ and using Taylor expansion
    we get,
    \begin{align*}
        d\calE[u](\varphi)
        &= \lim_{\epsilon \to 0} \frac{\calE(u + \epsilon \varphi) - \calE(u)}{\epsilon} = 0\\
        &= \lim_{\epsilon \to 0} \frac{\int_\Omega L(x, u + \epsilon \varphi, \nabla u + \epsilon \nabla \varphi) - f(x)\left(u(x) + \epsilon \varphi(x)\right) - L(x, u, \nabla u) + f(x)u(x) \; dx}{\epsilon}\\
        &= \lim_{\epsilon \to 0} \frac{\int_\Omega L(x, u, \nabla u) + \nbnbu L(x, u, \nabla u) \epsilon \nabla \varphi 
            +\nbu L(x, u, \nabla u)\epsilon u + r(x)- \epsilon f(x)\varphi(x) - L(x, u, \nabla u)\; dx }{\epsilon}
        \numberthis \label{eq:direction_der_pf_eq1}
        \end{align*}
    where for all $x \in \Omega$ we have,
    \begin{align*}
    |r(x)| &\leq 
        \frac{\epsilon^2}{2}\sup_{y \in \Omega} 
        \left|\left(\left(\nabla u(y)\right)^TD^2_{u(y)}L(y, u, \nabla u)\nabla u(y)\right)
        + \left(D^2_{u(y)} L(y, u(y), \nabla u(y)) u(y)^2\right)\right| \\
        &\leq \frac{\epsilon^2}{2} \left(\Lambda \|\nabla u(y)\|_2^2 + \varsigma \|u(y)\|_2^2\right)
        \numberthis \label{eq:direction_der_pf_eq2}
    \end{align*}
    Using results from \eqref{eq:direction_der_pf_eq1} and \eqref{eq:direction_der_pf_eq2} 
    and taking $\epsilon \to 0$,
    the derivative in the direction of $\varphi$
    is,
    \begin{align*}
        d\calE[u](\varphi) 
        &= \lim_{\epsilon \to 0} \frac{\int_\Omega  \nbnbu L(x, u, \nabla u) \nabla \varphi 
            +\nbu L(x, u, \nabla u)u - f(x)\varphi(x)\; dx}{\epsilon}
    \end{align*}
    Since $\epsilon \to 0$ the final derivative is of the form,
    \begin{equation}
        \label{eq:operator_in_normal form}
        d\calE[u](\varphi)
            =\int_\Omega \bigg(\nbnbu L(x, u, \nabla u) \nabla \varphi + 
                + \nbu L(x, u, \nabla v)\varphi - f \varphi\bigg) dx = 0.
    \end{equation}
    We will now use the following Green's Identity for functions $r, s \in \h$
    \begin{align*}
        \int_\Omega (\Delta r) s dx = - \int_\Omega \nabla r \cdot \nabla s dx + \int_{\partial \Omega} \frac{\partial u}{\partial n} v d \Gamma \\
        \implies \int_\Omega (\Delta r) s dx = - \int_\Omega \nabla r \cdot \nabla s dx  \numberthis 
        \label{eq:green_identity_final}
    \end{align*}
    where $n_i$ 
    is a normal at the boundary and 
    $d \Gamma$ is an infinitesimal element
    of the boundary $\partial \Omega$.
    
    Using the identity in \eqref{eq:green_identity_final} in \eqref{eq:operator_in_normal form}
    we get,
    \begin{align*}
        d\calE[u](\varphi) = \int_\Omega \bigg(-\nabla \cdot \left(\nbnbu L(x, u, \nabla u) \right)\varphi + \nbu L(x, u, \nabla u)\varphi - f\varphi\bigg) dx = 0\\
        \implies d\calE[u](\varphi) = \int_\Omega \bigg(-\divergence\left(\nbnbu L(x, u, \nabla u) \right)\varphi + \nbu L(x, u, \nabla u)\varphi - f\varphi\bigg) dx = 0\\
    \end{align*}
    
    
    That is the minima for the energy functional is reached at a $u$
    which solves the following PDE,
    $$d\calE(u) := -\divergence\left(\nbnbu L(x, u, \nabla u)\right) + \nbu L(x, u, \nabla u)= f.$$
    where we define $d\calE(\cdot)$ as the operator 
    $-\divergence\left(\nbnbu L(x, \cdot, \nabla \cdot)\right) + \nabla_{\cdot}L(x, \cdot, \nabla \cdot) $.

\end{proof}
